BYO: A Unified Framework for Benchmarking Large-Scale Graph Containers

A fundamental building block in any graph algorithm is a graph container - a data structure used to represent the graph. Ideally, a graph container enables efficient access to the underlying graph, has low space usage, and supports updating the graph efficiently. In this paper, we conduct an extensive empirical evaluation of graph containers designed to support running algorithms on large graphs. To our knowledge, this is the first apples-to-apples comparison of graph containers rather than overall systems, which include confounding factors such as differences in algorithm implementations and infrastructure. We measure the running time of 10 highly-optimized algorithms across over 20 different containers and 10 graphs. Somewhat surprisingly, we find that the average algorithm running time does not differ much across containers, especially those that support dynamic updates. Specifically, a simple container based on an off-the-shelf B-tree is only 1.22x slower on average than a highly optimized static one. Moreover, we observe that simplifying a graph-container Application Programming Interface (API) to only a few simple functions incurs a mere 1.16x slowdown compared to a complete API. Finally, we also measure batch-insert throughput in dynamic-graph containers for a full picture of their performance. To perform the benchmarks, we introduce BYO, a unified framework that standardizes evaluations of graph-algorithm performance across different graph containers. BYO extends the Graph Based Benchmark Suite (Dhulipala et al. 18), a state-of-the-art graph algorithm benchmark, to easily plug into different dynamic graph containers and enable fair comparisons between them on a large suite of graph algorithms. While several graph algorithm benchmarks have been developed to date, to the best of our knowledge, BYO is the first system designed to benchmark graph containers

==> abstract.tex <==
\begin{abstract}
  We introduce \apinameshort, a general graph-processing algorithm framework
  with the goal of standardizing evaluations of graph-algorithm performance
  across dynamic-graph containers.

  There has been significant effort devoted to developing efficient
  dynamic-graph containers (data structures) capable of supporting both graph
  analytics as well as changes to the graph. However, current experimental
  methodologies make it difficult to perform an apples-to-apples comparison of
  graph algorithm performance across different containers. To measure graph
  algorithm performance, dynamic-graph systems often directly implement a
  relatively small set of algorithms on top of the underlying graph
  container. Even if two empirical evaluations choose the same set of problems
  for comparison, the choice of algorithms to solve those problems as well as
  their implementations vary across systems. Therefore, it is hard to tell to
  what degree empirical speedups on algorithms come from improved graph
  containers or better algorithm implementations.

  On the other hand, graph-algorithm frameworks built on abstractions enable
  programmers to express a wide variety of graph algorithms with a set of
  primitives, which ideally would enable a direct comparison of containers that
  implement algorithms that connect to these frameworks via the
  primitives. However, existing framework implementations assume that the input
  graph is stored in the classical Compressed Sparse Row (CSR) representation
  for graphs for simplicity. As a result, these framework implementations are
  inflexible and difficult to adapt to arbitrary dynamic-graph containers.

  \apinameshort extends the Graph Based Benchmark Suite (Dhulipala et al. 18), a
  state-of-the-art abstraction for implementing graph algorithms, to easily plug
  into dynamic graph containers to enable fair comparisons between them. One of
  the main goals of \apinameshort is to enable graph-container developers to
  easily test their data structures' performance on a large suite of graph
  algorithms without much additional programming effort.  To demonstrate the
  applicability of \apinameshort, we conduct a large-scale benchmarking study by
  connecting \numdatastructures graph containers to \apinameshort, which enables
  us to evaluate them on a suite of \numalgorithms graph algorithms. To the best
  of our knowledge, this is the first such apples-to-apples study of dynamic
  graph containers.\todo{should we add some more evaluation summary?}
\kuba{Revised version below}
%Designing a high-performance graph container is a challening task, 
A fundamental building block in any graph algorithm is a \emph{graph container} -- a data structure used to represent the graph.
Ideally, a graph container enables efficient read access and updates to the underlying graph.
In this paper, we conduct an extensive empirical evaluation of graph containers designed to support running algorithms on large graphs.

We measure the running time of 10 highly-optimized algorithms across over 20 different containers and 10 graphs.
Somewhat surprisingly, we find that the average algorithm running time does not differ much across containers, especially those that support dynamic updates.
Specifically, a simple container based on an off-the-shelf B-tree is only X\% slower than a highly optimized one.
Moreover, we observe that simplifying a graph container API to only 2 simple functions incurs a mere Y\% slowdown compared to ...
Our results indicate that the main distinguishing factor between different graph containers is the update throughput, which may vary as much as Z\% between ...

To perform the benchmarks, we introduce \apinameshort, a general graph-processing algorithm framework standardizing evaluations of graph-algorithm performance across dynamic-graph containers.
\apinameshort extends the Graph Based Benchmark Suite (Dhulipala et al. 18), a
state-of-the-art graph algorithm benchmark, to easily plug into different dynamic graph containers and enable fair comparisons between them on a large suite of graph algorithms.
While several graph algorithm benchmarks have been developed to date, to the best of our knowledge \apinameshort is the first system designed to benchmark graph containers.
\end{abstract}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> api_comparison.tex <==
\subsection{API Comparison}



==> cover_page.tex <==
\begin{titlepage}
    \twocolumn[{%
     \centering \bf
     \LARGE Revision Summary: 
     BYO: A Unified Framework for Benchmarking Large-Scale Graph Containers [Experiment, Analysis \& Benchmark] \\[1.5em]
    }]

We are submitting a revised version of our manuscript “BYO: A Unified Framework for Benchmarking Large-Scale Graph Containers” to VLDB 2024.

We have addressed all of the required changes requested by the reviewers. Detailed explanations of how we address the reviewers’ requests appear following the cover letter. We have color coded all our changes corresponding to reviewer comments. Changes in the text appear in blue and new content is green colored. We also use margin markers to refer to the specific comments. 

\todo{[FILLIN HIGH-LEVEL OF WHAT WE DID]}

We thank the reviewers for their comments. The paper is much improved due to their feedback.

\begin{tcolorbox}
    \textbf{Reivewer \#1 D1.} The paper is very well written and convincingly motivates the problem. However, some important information is somewhat hidden in the background section, e.g., the supported types of graphs.
\end{tcolorbox}
We have expanded BYO’s capabilities to support directed/undirected graphs as well as weighted/unweighted graphs.
To make this information more prominent, we have moved it to \cref{sec:intro} (at the top of page 2): “For generality, BYO is able to represent directed and undirected graphs, as well as weighted and unweighted graphs.”

\begin{tcolorbox}
    \textbf{Reivewer \#1 D2.} A detailed discussion summarization of what characteristics of which container to use in combination with which algorithm and dataset characteristics would be interesting to have.
\end{tcolorbox}
xxx

\begin{tcolorbox}
    \textbf{Reivewer \#1 D3.} The truly assess all the effort that led to this paper, it would be interesting to know how much the extended tools and libraries already deliver and what the extension for this paper was.
\end{tcolorbox}
xxx

\begin{tcolorbox}
    \textbf{Reivewer \#4 D1.} The motivation of comparing different graph containers should be further justified. On one hand, there are many factors to influence the running time of a graph algorithm such as the complexity of the problem itself, algorithm implementation, the design of the system, scheduling, complier, parallelization methods, etc. Among them, the graph container may not be one of most influential factors or bottlenecks w.r.t performance. Furthermore, for those complex graph algorithms, it is the auxiliary data structure (or index) that determines the efficiency, not the graph data structures itself. On the other hand, from the results, the difference of performance over difference containers is relatively small, which undermines the importance of the evaluation. To justify the importance of containers, the time percentage of graph access/update time to the whole running time of various categories of graph applications should be tested.
\end{tcolorbox}
xxx

\begin{tcolorbox}
    \textbf{Reivewer \#4 D2.} The BYO API only covers a subset of general graph operations. Some other important operations such as set intersection, common neighbors, are missing, which limited the scope of tested applications, such as triangle counting, k-truss community, bipartite graph problems, structural similarities, etc.
\end{tcolorbox}
xxx

\begin{tcolorbox}
    \textbf{Reivewer \#4 D3.} Why the performance over containers is measured based on the ratio to the CSR results, instead of directly comparing the performance, should be discussed, if CSR is not the benchmark or standardization in the literature. For example, Figure 2 is measured by the ratio to CSR while Figure 3 measures the running time directly, and in Figure 7, the results are normalized to BYO, this loses consistence.
\end{tcolorbox}
xxx

\begin{tcolorbox}
    \textbf{Reivewer \#4 D4.} The experiments do not test the space usage of different containers, which is also important for large graphs.
\end{tcolorbox}
xxx

\begin{tcolorbox}
    \textbf{Reivewer \#4 D5.} The related works can be improved by including more discussions about pros and cons of different containers in the literature.
\end{tcolorbox}
xxx

\begin{tcolorbox}
    \textbf{Reivewer \#4 D6.} As for the testing of dynamic scenarios, it is usually not updating the graphs matters, but the update of the index of different dynamic graph algorithms. Indeed, most of the algorithms listed in Table 3 have a dynamic version (incremental algorithm), only testing updating the containers and ignoring their effects on the running time of the incremental algorithms undermines the usability of the results.
\end{tcolorbox}
xxx

\begin{tcolorbox}
    \textbf{Reivewer \#4 D7.} As for the experimental results, the relatively small difference of the performance over different graph containers shows little guidance for the further research as a experimental paper. It would be better the author can map different containers to different categories of graph applications or scenarios, for better choosing among containers.
\end{tcolorbox}
xxx

\begin{tcolorbox}
    \textbf{Reivewer \#5 D1.} The technical challenge of this paper needs to be clarified. The paper proposed a framework BYO, which is a translation layer on top of GBBS. The technical part presented several APIs implemented in BYO. Other than identifying and implementing these APIs, the technical contribution is limited. The challenges of integrating BYO with GBBS would need to be clarified for better understanding.
\end{tcolorbox}
xxx

\begin{tcolorbox}
    \textbf{Reivewer \#5 D2.} The result of this experiment indicates that special-purposed graph containers generally perform better than off-the-shelf containers on most tasks, especially in worst-case performance. This result is somewhat expected from the common sense of a researcher in the field, as one would expect this kind of result with relatively simple reasoning and analysis. The motivation for conducting such an experiment is less convincing.
\end{tcolorbox}
xxx

\begin{tcolorbox}
    \textbf{Reivewer \#5 D3.} The reason for selecting GBBS as the base of BYO implementation needs to be explained. More explanation on the selection of implementation choices will help.
\end{tcolorbox}
xxx



\end{titlepage}
\pagenumbering{arabic}

==> figures/how_close_api.tex <==
\begin{figure}
    \centering
\begin{tikzpicture}
\small
\begin{axis}[
  xlabel= Slowdown over Full API,
  ylabel style={align=center},
  ylabel= Percent of Experiments\\ Within Slowdown,
  ymax = 100,
  ymin = 0,
  xmax=2,
  xmin=1,
  legend columns=3,
  legend style={at={(.98,1)},anchor=south east},
  legend style={font=\footnotesize},
  width=\linewidth, height=3.5cm,
  legend style={inner xsep=0pt, inner ysep=0pt},
         ]

\addplot +[mark=none, loosely dashdotted, very thick, safe-peach ] table [x=slowdown, y=run_min, col sep=tab] {tsvs/how_close_api.tsv};
\addlegendentry{Min}
\addplot +[mark=none, dotted, very thick, safe-teal] table [x=slowdown, y=run_min_efficient, col sep=tab] {tsvs/how_close_api.tsv};
\addlegendentry{Min efficient}
\addplot +[mark=none, dash pattern=on \pgflinewidth off 5pt, very thick, safe-pink] table [x=slowdown, y=run_no_early_exit, col sep=tab] {tsvs/how_close_api.tsv};
\addlegendentry{No early exit}
\addplot +[mark=none, dash pattern=on \pgflinewidth off .5pt, very thick, safe-plum] table [x=slowdown, y=run_no_parallel_map, col sep=tab] {tsvs/how_close_api.tsv};
\addlegendentry{No parallel map}
\addplot +[mark=none, densely dashdotted, very thick, safe-green] table [x=slowdown, y=run_just_degree, col sep=tab] {tsvs/how_close_api.tsv};
\addlegendentry{Min + \degree}
\end{axis}
\end{tikzpicture}
    \caption{Slowdown of different API configurations compared to the full API using CSR.
    % as the underlying container.
    \tabref{api-components-avg} describes the API configurations and~\secref{byo-api} specifies the required and optional functionality in \apinameshort.
    Each point $(x, y)$ for a given API configuration means that the configuration was at most $x$ times slower than the full API on $y\%$ of experiments.
   A line going up faster implies that that configuration achieves closer performance relative to the full API on more experiments. We find that the minimal map functionality with \degree and \numedges are enough to get good performance on most experiments.}
    \label{fig:how_close_api}
\end{figure}

\iffalse
\begin{figure}
    \centering
\begin{tikzpicture}
\begin{axis}[
  xlabel= Slowdown over CSR,
  ylabel style={align=center},
  ylabel= Percent of Experiments\\ Within Slowdown,
  ymax = 100,
  ymin = 0,
  xmax=2,
  xmin=1,
  legend columns=2,
  legend style={at={(.98,.8)},anchor=north east},
  legend style={font=\footnotesize},
  width=8cm, height=5cm,
         ]

\addplot +[mark=none, loosely dashdotted, very thick, safe-peach ] table [x=slowdown, y=run_dhb, col sep=tab] {tsvs/how_close_structures.tsv};
\addlegendentry{DHB}
\addplot +[mark=none, dotted, very thick, safe-teal] table [x=slowdown, y=run_sstgraph, col sep=tab] {tsvs/how_close_structures.tsv};
\addlegendentry{SSTGraph}
\addplot +[mark=none, dash pattern=on \pgflinewidth off 5pt, very thick, safe-pink] table [x=slowdown, y=run_absl_btree_set_inplace, col sep=tab] {tsvs/how_close_structures.tsv};
\addlegendentry{B-tree}
\addplot +[mark=none, dash pattern=on \pgflinewidth off .5pt, very thick, safe-plum] table [x=slowdown, y=run_terrace, col sep=tab] {tsvs/how_close_structures.tsv};
\addlegendentry{Terrace}
\addplot +[mark=none, dash pattern=on 3pt off 1pt, very thick, safe-orange] table [x=slowdown, y=run_single_pma, col sep=tab] {tsvs/how_close_structures.tsv};
\addlegendentry{PMA}
\addplot +[mark=none, dash pattern=on 3pt off 7pt, very thick, safe-brick] table [x=slowdown, y=run_vector_aspen_inplace, col sep=tab] {tsvs/how_close_structures.tsv};
\addlegendentry{Aspen}
\addplot +[mark=none, densely dashdotted, very thick, safe-green] table [x=slowdown, y=run_std_set_inplace, col sep=tab] {tsvs/how_close_structures.tsv};
\addlegendentry{std::set}
\addplot +[mark=none, solid, safe-black, thick] table [x=slowdown, y=run_vector_cpam_inplace, col sep=tab] {tsvs/how_close_structures.tsv};
\addlegendentry{CPAM}
\end{axis}
\end{tikzpicture}
    \caption{How many different experiments (a specific algorithm on a particular graph) each graph container incurred at most $x$ slowdown of CSR.  A line going up faster implies that the container achieves closer performance relative to CSR on more experiments.  We find that almost all structures are able to perform the majority of the experiments with at most a $1.4\times$ slowdown over CSR.}
    \label{fig:how_close_structures}
\end{figure}
\fi

==> figures/insert_no_sort.tex <==
\begin{figure}
    \centering
\begin{tikzpicture}
\begin{axis}[
  xlabel= Batch Size,
  ylabel style={align=center},
  ylabel= Throughput \\ (edges per second),
  xmin=10,
  xmax=100000000,
  legend columns=3,
  legend style={at={(1,1)},anchor=south east},
    legend style={font=\tiny, row sep=0pt},
  xmode=log,
  width=\linewidth, height=4cm,
         ]
\addplot +[mark=none, densely dashdotted, very thick, safe-green] table [x=batch_size, y=run_std_set_inplace, col sep=tab] {tsvs/insert_no_sort.tsv};
\addlegendentry{\stdset}
\addplot +[mark=none, dash pattern=on \pgflinewidth off 5pt, very thick, safe-pink] table [x=batch_size, y=run_absl_btree_set_inplace, col sep=tab] {tsvs/insert_no_sort.tsv};
\addlegendentry{\abslbtree}
\addplot +[mark=none, dash pattern=on 3pt off 7pt, very thick, safe-brick] table [x=batch_size, y=run_absl_flat_hash_set_inplace, col sep=tab] {tsvs/insert_no_sort.tsv};
\addlegendentry{\abslflathash}
\addplot +[mark=none, solid, safe-black, thick] table [x=batch_size, y=run_vector_cpam_inplace, col sep=tab] {tsvs/insert_no_sort.tsv};
\addlegendentry{CPAM}
\addplot +[mark=none, loosely dashdotted, very thick, safe-peach ] table [x=batch_size, y=run_dhb, col sep=tab] {tsvs/insert_no_sort.tsv};
\addlegendentry{DHB}
\addplot +[mark=none, dotted, very thick, safe-teal] table [x=batch_size, y=run_sstgraph, col sep=tab] {tsvs/insert_no_sort.tsv};
\addlegendentry{SSTGraph}
\addplot +[mark=none, dash pattern=on \pgflinewidth off .5pt, very thick, safe-plum] table [x=batch_size, y=run_terrace, col sep=tab] {tsvs/insert_no_sort.tsv};
\addlegendentry{Terrace}
\addplot +[mark=none, dash pattern=on 3pt off 1pt, very thick, safe-orange] table [x=batch_size, y=run_single_pma, col sep=tab] {tsvs/insert_no_sort.tsv};
\addlegendentry{PMA}
\end{axis}
\end{tikzpicture}
    \caption{The throughput of inserts for different batch sizes.  We do not
      include the cost to sort the batch, which every data structure needs to do
      in some way to be able to insert efficiently in parallel. Of the data
      structures in this plot, \stdset, \abslbtree, and \abslflathash are
      off-the-shelf containers, while the others are optimized. Details about
      the different graph containers can be found in Section
      \ref{sec:datastr}.\todo{update with new numbers}}
    \label{fig:inserts_no_sort}
\end{figure}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> tables/api-comparison-tables.tex <==



\begin{table*}[t]
  \centering
 % \resizebox{\linewidth}{!}{%
  \begin{tabular}{@{}llrrrrrrrrrrrrrr@{}}
    \toprule
    \textit{System}   & \textit{Problem}   & \textit{\roadshort}       &  \textit{\ljshort} & \textit{\orkutshort} &
                                                                                                                     \textit{\rmatshort}  &  \textit{\ershort} & \textit{\proteinshort}
    & \textit{\twittershort}  &  \textit{\papersshort} & \textit{\friendstershort}
    & \textit{\kronshort}   \\
    \midrule
    GAP &BFS&0.49&0.01&0.01&0.02&0.03&0.01&0.11&0.28&0.22&0.08\\
                      &BC&0.66&0.06&0.08&0.31&1.72&0.11&1.96&3.23&2.96&0.61\\
                      &CC&0.03&0.01&0.01&0.02&0.03&0.15&0.09&0.33&0.21&0.22\\
                      &PR&0.14&0.17&0.37&0.61&0.45&2.02&4.85&16.82&17.08&4.27\\
    \bottomrule
    GraphBLAS  &BFS&2.80&0.23&0.21&0.25&0.27&1.27&0.46&0.90&0.63&0.38\\
                      &BC&6.34&0.98&0.58&1.26&1.00&1.95&1.98&4.38&3.44&4.40\\
                      &CC&1.94&0.48&0.29&0.66&0.64&4.08&1.24&2.29&1.85&1.43\\
                      &PR&1.58&0.84&0.80&1.43&0.77&6.29&11.25&21.42&22.97&14.13\\
    \bottomrule
    Ligra  &BFS&1.02&0.01&0.01&0.03&0.03&0.02&0.12&0.41&0.33&0.17\\
                      &BC&2.23&0.05&0.05&0.10&0.15&0.08&0.79&2.41&2.18&2.22\\
                      &CC&12.80&0.05&0.05&0.12&0.52&0.79&1.36&5.46&4.01&3.54\\
                      &PR&0.58&0.51&1.04&2.44&2.25&12.80&28.10&61.30&68.20&22.80\\

    \bottomrule
    GBBS&BFS&1.70&0.01&0.02&0.02&0.04&0.02&0.10&0.37&0.29&0.17\\
                      &BC&3.31&0.04&0.06&0.15&0.24&0.23&0.83&2.52&2.30&2.86\\
                      &CC&0.02&0.02&0.03&0.07&0.15&0.18&0.64&1.49&1.49&1.47\\
                      &PR&0.56&0.21&0.31&0.69&0.62&3.34&9.52&21.90&22.58&7.69\\
    \bottomrule
    \apinameshort &BFS&0.59&0.01&0.01&0.01&0.02&0.02&0.08&0.27&0.20&0.12\\
&BC&4.05&0.04&0.05&0.16&0.24&0.22&0.99&2.60&2.35&2.69\\
&CC&0.03&0.02&0.03&0.09&0.18&0.21&0.70&1.96&1.67&1.58\\
&PR&0.57&0.22&0.34&0.96&0.65&2.73&10.16&20.60&19.85&8.07\\
    \bottomrule
  \end{tabular}
 % }
  \caption{Time (in seconds) to perform algorithms in different graph-processing
    libraries.\helen{maybe we can cut this for space}}
  \label{tab:frameworks-performance}
\end{table*}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> tables/api_descriptions.tex <==
\iffalse
\begin{table}[t]
  \centering
    \resizebox{\linewidth}{!}{%
  \begin{tabular}{@{}lrrrrrr@{}}
    \toprule
    \textit{Framework} & \textit{Type} & \textit{Programming abstraction} \\
    \midrule
    \textit{\apinameshort}  &  \begin{tabular}{@{}r@{}} High-level \\
                                 framework\end{tabular}  & \begin{tabular}{@{}r@{}}VertexSubset/Bucketing/ \\
                                                             Vertex/Graph\end{tabular} \\
    \textit{GBBS}  &  \begin{tabular}{@{}r@{}} High-level \\
                        framework\end{tabular} &  \begin{tabular}{@{}r@{}}VertexSubset/Bucketing/ \\
                                                    Vertex/Graph\end{tabular} \\
    \textit{Ligra}  & \begin{tabular}{@{}r@{}} High-level \\
                        framework\end{tabular}& VertexSubset/EdgeMap \\
    \textit{GraphBLAS}& \begin{tabular}{@{}r@{}} High-level \\
                          framework\end{tabular} & Sparse linear algebra \\
    \textit{GAP} & \begin{tabular}{@{}r@{}}Direct \\
                     implementation\end{tabular} & Vertex-centric \\
    \bottomrule
  \end{tabular}
  }
  \caption{Graph systems included in the evaluation and their implementation
    descriptions.\todo{check it}\helen{also we might cut this for space}}
  \label{tab:frameworks-description}
\end{table}


\begin{table}[t]
  \centering
 % \resizebox{\linewidth}{!}{%
  \begin{tabular}{@{}lrrr@{}}
    \toprule
    \textit{Problem}  &  \textit{\apinameshort/GBBS/Ligra} &  \textit{GraphBLAS} & \textit{GAP} \\
    \midrule
    BFS & \begin{tabular}{@{}r@{}}Direction- \\
            optimizing~\cite{BeamerAsPa12}\end{tabular}& \begin{tabular}{@{}r@{}}Direction- \\
                                       optimizing\end{tabular} &
                                                    \begin{tabular}{@{}r@{}}Direction- \\
                                                      optimizing\end{tabular}
    \\
    BC & Brandes~\cite{Brandes01}  & Brandes &  Brandes  \\
    CC & Union-find~\cite{SimsiriTaTi16} & FastSV~\cite{ZhangAzHu20} & Afforest~\cite{SuttonBeBa18} \\
    PR & Jacobi SpMV & Jacobi SpMV & Jacobi SpMV \\
    \bottomrule
  \end{tabular}
 % }
  \caption{Underlying algorithms for the tested common problems across graph
    systems.\helen{can someone check the cite for Union-find (CC) for BYO/GBBS?}\todo{cut this and just say it in the text}}
  \label{tab:frameworks-algorithms}
\end{table}
\fi
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> tables/data-structure-descriptions.tex <==

\begin{table*}[t]
\footnotesize
  \centering
  \begin{tabular}{@{}lrrrrrrr@{}}
    \toprule
    \textit{Container} &  \begin{tabular}{@{}r@{}} 
                            \textit{Underlying data structure(s)}  \end{tabular}
    &   \\
    \midrule
    \textit{\setapi{} (Vector of ...)} & & \textit{Size} & \textit{Iterator} & \textit{Map} & \begin{tabular}{@{}r@{}} \textit{Map with} \\
                            \textit{early exit}  \end{tabular} &  \textit{Parallel map}  & \begin{tabular}{@{}r@{}} \textit{Parallel Map} \\
                            \textit{ with early exit}  \end{tabular} \\
    \midrule
    \stdvector~\cite{MusserDeSa01, Josuttis12}
                       & Array & \Checkmark & \xmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark \\
    \stdset~\cite{MusserDeSa01, Josuttis12} & Binary search tree &  \Checkmark  & \Checkmark & (\Checkmark)
                                       & (\Checkmark) & \xmark & \xmark\\

    \stdunorderedset~\cite{MusserDeSa01, Josuttis12} & Node Hash table &  \Checkmark  & \Checkmark &  (\Checkmark) & (\Checkmark) & \xmark & \xmark \\
    \abslbtree~\cite{absl} & B-tree &  \Checkmark   & \Checkmark &
                                                                       (\Checkmark)
                                       &  (\Checkmark) & \xmark & \xmark\\
    \abslflathash~\cite{absl} & Flat hash map & \Checkmark & \Checkmark &  (\Checkmark) &  (\Checkmark)& \xmark & \xmark \\
    Aspen$^\dagger$ ~\cite{DhulipalaBlSh19} & C-tree & \Checkmark & \xmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark  \\
   CPAM$^\dagger$ ~\cite{DhulipalaBlGu22} & PaC-tree &
                                                                                \Checkmark & \xmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark \\
     Tinyset~\cite{WheatmanBu21} & PMA &
                                                                                \Checkmark & \xmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark \\
    PMA$^\dagger$ ~\cite{WheatmanBuBu23} & PMA &
                                                                                \Checkmark & \xmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark \\
    \midrule
    \textit{\containerapi{}} & & \textit{Degree} & \textit{Num\_edges} & \textit{Map} & \begin{tabular}{@{}r@{}} \textit{Map with} \\
                            \textit{early exit}  \end{tabular} &  \textit{Parallel map}  & \begin{tabular}{@{}r@{}} \textit{Parallel map} \\
                            \textit{with early exit}  \end{tabular} \\
    \midrule
    CSR$^\dagger$ ~\cite{TinneyWa67} & Array & \Checkmark & \Checkmark & \Checkmark & \Checkmark & \Checkmark  & \Checkmark \\
    SSTGraph~\cite{WheatmanBu21} & Tinyset &  \Checkmark & (\xmark) & \Checkmark & \Checkmark & \Checkmark  & \Checkmark\\
    Terrace~\cite{PandeyWhXu21} & Array, PMA, B-tree & \Checkmark & \Checkmark & \Checkmark & \Checkmark &
                                                                     \Checkmark &\Checkmark\\
    DHB~\cite{VanPrWi22} & Hash blocks & \Checkmark & (\xmark) & \Checkmark & \Checkmark & \xmark & \xmark \\
    PMA$^\dagger$ ~\cite{WheatmanBuBu23} & PMA & (\xmark) & (\xmark) &  \Checkmark &  \Checkmark &
                                                                             \Checkmark
    &  \Checkmark\\
    \bottomrule
  \end{tabular}
  
  \caption{Description of all of the tested container types and which parts of
    the \apinameshort API they or their wrappers (connections between the container and \apinameshort) implement. A \Checkmark means the data structure
    implements it directly and an \xmark means the data structure does not
    implement it. A (\Checkmark) means the function is provided via
    \apinameshort's translation layer. An (\xmark) means the function is
    unimplemented but the metadata is maintained at the framework level
    (\secref{byo-metadata}). Data structures with both uncompressed and compressed versions have a $^\dagger$ mark next to them. The \setapi version of \stdvector is a special case where the wrapper implements all required mapping functions directly instead of using the automatic translation between the iterator and map as an example of how to implement the different functions.}
  \label{tab:data-structure-descriptions}
\end{table*}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> tables/data-structures-tables.tex <==

\begin{table*}
\begin{tabular}{lrrrrrrrrrr}
\toprule
 & RD & LJ & CO & RM & ER & PR & TW & PA & FS & KR \\
system &  &  &  &  &  &  &  &  &  &  \\
\midrule
absl\_btree\_set & 1.12 & 1.24 & 1.30 & 1.27 & 1.36 & 1.14 & 1.43 & 1.19 & 1.17 & 1.37 \\
absl\_btree\_set\_inplace & 1.07 & 1.17 & 1.28 & 1.18 & 1.24 & 1.15 & 1.43 & 1.08 & 1.17 & 1.49 \\
absl\_flat\_hash\_set & 1.22 & 1.46 & 1.68 & 1.50 & 1.33 & 1.29 & 1.76 & 1.21 & 1.23 & 1.46 \\
absl\_flat\_hash\_set\_inplace & 1.03 & 1.28 & 1.40 & 1.28 & 1.27 & 1.29 & 1.68 & 1.19 & 1.20 & 1.41 \\
csr & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
csr\_byte & 1.00 & 1.02 & 1.03 & 1.05 & 1.03 & 1.04 & 1.04 & 1.12 & 1.09 & 1.05 \\
csr\_compressed & 1.14 & 1.22 & 1.27 & 1.30 & 1.21 & 1.29 & 1.20 & 1.25 & 1.24 & 1.22 \\
csr\_shuffled & 1.02 & 1.05 & 1.11 & 1.00 & 1.01 & 1.00 & 1.04 & 0.98 & 1.02 & 1.02 \\
dhb & 1.03 & 1.24 & 1.25 & 1.19 & 1.11 & 1.06 & 1.35 & 1.07 & 1.07 & 1.16 \\
single\_cpma & 1.08 & 1.38 & 1.43 & 1.39 & 1.33 & 1.43 & 1.29 & 1.29 & 1.27 & 1.22 \\
single\_pma & 1.04 & 1.15 & 1.18 & 1.22 & 1.16 & 1.19 & 1.17 & 1.14 & 1.13 & 1.13 \\
single\_scpma & 1.10 & 1.40 & 1.47 & 1.46 & 1.36 & 1.45 & 1.30 & 1.29 & 1.27 & 1.24 \\
single\_spma & 1.05 & 1.16 & 1.21 & 1.25 & 1.20 & 1.24 & 1.17 & 1.16 & 1.14 & 1.16 \\
sstgraph & 1.10 & 1.26 & 1.25 & 1.29 & 1.17 & 1.27 & 1.41 & 1.19 & 1.21 & 1.33 \\
std\_set & 1.43 & 2.55 & 3.11 & 3.10 & 3.11 & 3.45 & 3.11 & 2.22 & 2.14 & 2.42 \\
std\_set\_inplace & 1.05 & 2.31 & 2.98 & 2.82 & 2.89 & 3.45 & 2.99 & 1.88 & 2.02 & 2.38 \\
std\_unordered\_set & 1.57 & 2.06 & 2.76 & 2.42 & 1.98 & 2.20 & 2.21 & 1.70 & 1.83 & 1.64 \\
std\_unordered\_set\_inplace & 1.41 & 1.85 & 2.47 & 2.19 & 1.96 & 2.22 & 2.14 & 1.64 & 1.77 & 1.63 \\
terrace & 1.08 & 1.13 & 1.31 & 1.11 & 1.04 & 1.13 & 1.59 & 1.10 & 1.15 & 1.47 \\
vector\_aspen & 1.38 & 1.21 & 1.15 & 1.18 & 1.17 & 1.13 & 1.25 & 1.17 & 1.19 & 1.38 \\
vector\_aspen\_inplace & 1.10 & 1.10 & 1.12 & 1.11 & 1.11 & 1.15 & 1.16 & 1.14 & 1.18 & 1.21 \\
vector\_compressed\_aspen & 1.27 & 1.32 & 1.50 & 1.54 & 1.49 & 1.52 & 1.48 & 1.46 & 1.42 & 1.45 \\
vector\_compressed\_aspen\_inplace & 1.08 & 1.25 & 1.42 & 1.38 & 1.33 & 1.52 & 1.37 & 1.30 & 1.36 & 1.43 \\
vector\_compressed\_cpam & 1.27 & 1.31 & 1.42 & 1.48 & 1.36 & 1.49 & 1.32 & 1.39 & 1.38 & 1.29 \\
vector\_compressed\_cpam\_inplace & 1.09 & 1.21 & 1.31 & 1.31 & 1.27 & 1.49 & 1.31 & 1.24 & 1.36 & 1.46 \\
vector\_cpam & 1.23 & 1.24 & 1.12 & 1.16 & 1.11 & 1.17 & 1.13 & 1.14 & 1.16 & 1.11 \\
vector\_cpam\_inplace & 1.08 & 1.12 & 1.09 & 1.08 & 1.04 & 1.18 & 1.12 & 1.07 & 1.19 & 1.16 \\
vector\_cpma & 1.60 & 1.54 & 1.40 & 1.43 & 1.24 & 1.23 & 1.31 & 1.30 & 1.23 & 1.26 \\
vector\_pma & 1.60 & 1.40 & 1.24 & 1.27 & 1.10 & 1.13 & 1.24 & 1.23 & 1.17 & 1.19 \\
vector\_scpma & 1.60 & 1.53 & 1.43 & 1.40 & 1.24 & 1.24 & 1.33 & 1.29 & 1.23 & 1.25 \\
vector\_spma & 1.60 & 1.46 & 1.25 & 1.28 & 1.10 & 1.12 & 1.24 & 1.24 & 1.18 & 1.17 \\
vector\_tinyset & 1.14 & 1.20 & 1.32 & 1.22 & 1.17 & 1.12 & 1.74 & 1.12 & 1.16 & 1.71 \\
vector\_vector & 1.13 & 1.03 & 1.03 & 1.08 & 1.01 & 1.05 & 1.07 & 1.07 & 1.11 & 1.16 \\
\bottomrule
\end{tabular}
\caption{\brian{performance on different graphs averaged across all algorithms}}
\label{tab:datastr-over-algs}
\end{table*}

\begin{table*}
\begin{tabular}{lrrrrrrrrrr}
\toprule
 & BFS & BC & Spanner & LDD & CC & WEDS & KCore & Coloring & MIS & PR \\
system &  &  &  &  &  &  &  &  &  &  \\
\midrule
absl\_btree\_set & 1.49 & 1.35 & 1.14 & 1.42 & 0.98 & 1.26 & 1.25 & 1.30 & 1.24 & 1.20 \\
absl\_btree\_set\_inplace & 1.33 & 1.26 & 1.11 & 1.24 & 0.96 & 1.27 & 1.30 & 1.40 & 1.20 & 1.20 \\
absl\_flat\_hash\_set & 1.72 & 1.51 & 1.36 & 1.66 & 1.20 & 1.32 & 1.24 & 1.44 & 1.33 & 1.33 \\
absl\_flat\_hash\_set\_inplace & 1.43 & 1.39 & 1.14 & 1.38 & 1.03 & 1.35 & 1.20 & 1.50 & 1.29 & 1.30 \\
csr & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 \\
csr\_byte & 1.15 & 1.02 & 1.03 & 1.10 & 0.99 & 1.09 & 1.01 & 1.01 & 1.07 & 0.99 \\
csr\_compressed & 1.23 & 1.34 & 1.28 & 1.22 & 1.23 & 1.19 & 1.04 & 1.23 & 1.31 & 1.30 \\
csr\_shuffled & 1.06 & 1.04 & 1.12 & 1.07 & 0.86 & 1.06 & 1.01 & 1.04 & 0.99 & 1.03 \\
dhb & 1.40 & 1.11 & 1.05 & 1.28 & 0.90 & 1.14 & 1.19 & 1.22 & 1.16 & 1.10 \\
single\_cpma & 1.39 & 1.48 & 1.28 & 1.19 & 1.12 & 1.22 & 1.04 & 1.40 & 1.38 & 1.72 \\
single\_pma & 1.33 & 1.22 & 1.17 & 1.22 & 1.05 & 1.11 & 1.03 & 1.03 & 1.17 & 1.20 \\
single\_scpma & 1.41 & 1.52 & 1.29 & 1.21 & 1.13 & 1.23 & 1.05 & 1.43 & 1.39 & 1.76 \\
single\_spma & 1.36 & 1.27 & 1.18 & 1.27 & 1.09 & 1.12 & 1.04 & 1.04 & 1.18 & 1.21 \\
sstgraph & 1.26 & 1.27 & 1.25 & 1.22 & 1.21 & 1.18 & 1.06 & 1.56 & 1.20 & 1.32 \\
std\_set & 3.27 & 3.55 & 2.37 & 2.69 & 2.25 & 2.36 & 1.69 & 2.32 & 2.98 & 2.96 \\
std\_set\_inplace & 2.63 & 3.31 & 2.20 & 2.17 & 2.09 & 2.33 & 1.61 & 2.22 & 2.73 & 2.77 \\
std\_unordered\_set & 3.00 & 2.31 & 1.95 & 2.82 & 1.58 & 1.75 & 1.34 & 1.70 & 2.15 & 2.05 \\
std\_unordered\_set\_inplace & 2.59 & 2.25 & 1.85 & 2.26 & 1.50 & 1.71 & 1.34 & 1.76 & 2.09 & 2.00 \\
terrace & 1.34 & 1.12 & 1.26 & 1.32 & 1.01 & 1.23 & 1.20 & 1.38 & 1.10 & 1.09 \\
vector\_aspen & 1.37 & 1.11 & 1.10 & 1.38 & 0.90 & 1.23 & 1.26 & 1.68 & 1.16 & 1.13 \\
vector\_aspen\_inplace & 1.13 & 1.06 & 1.04 & 1.14 & 1.01 & 1.17 & 1.12 & 1.64 & 1.10 & 1.05 \\
vector\_compressed\_aspen & 1.44 & 1.64 & 1.31 & 1.40 & 1.17 & 1.46 & 1.16 & 1.91 & 1.49 & 1.60 \\
vector\_compressed\_aspen\_inplace & 1.21 & 1.46 & 1.25 & 1.22 & 1.19 & 1.39 & 1.08 & 1.86 & 1.41 & 1.45 \\
vector\_compressed\_cpam & 1.45 & 1.51 & 1.34 & 1.37 & 1.25 & 1.33 & 1.04 & 1.56 & 1.44 & 1.47 \\
vector\_compressed\_cpam\_inplace & 1.18 & 1.36 & 1.26 & 1.18 & 1.27 & 1.38 & 1.14 & 1.59 & 1.33 & 1.39 \\
vector\_cpam & 1.22 & 1.14 & 1.09 & 1.18 & 1.03 & 1.20 & 1.10 & 1.39 & 1.12 & 1.12 \\
vector\_cpam\_inplace & 1.11 & 1.04 & 1.05 & 1.12 & 1.00 & 1.17 & 1.08 & 1.42 & 1.10 & 1.09 \\
vector\_cpma & 1.55 & 1.38 & 1.33 & 1.52 & 1.23 & 1.29 & 1.14 & 1.27 & 1.43 & 1.38 \\
vector\_pma & 1.51 & 1.20 & 1.22 & 1.49 & 1.11 & 1.23 & 1.07 & 1.18 & 1.32 & 1.25 \\
vector\_scpma & 1.58 & 1.38 & 1.33 & 1.52 & 1.23 & 1.29 & 1.14 & 1.27 & 1.42 & 1.39 \\
vector\_spma & 1.55 & 1.20 & 1.22 & 1.49 & 1.11 & 1.22 & 1.07 & 1.18 & 1.32 & 1.28 \\
vector\_tinyset & 1.38 & 1.26 & 1.24 & 1.34 & 1.21 & 1.28 & 1.24 & 1.56 & 1.14 & 1.15 \\
vector\_vector & 1.14 & 0.97 & 0.93 & 1.16 & 1.23 & 1.12 & 1.09 & 1.08 & 1.07 & 0.98 \\
\bottomrule
\end{tabular}
\caption{\brian{performance on different algorithms averaged across all graphs}}
\label{tab:datastr-over-graphs}
\end{table*}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

